Modeling E-Bike Route Choice in Washington, DC: A Path Size Logit Approach

Understanding e-bike route choice is essential for developing effective cycling infrastructure, yet empirical evidence remains limited. This study investigates shared e-bike route choice in Washington, DC, using Global Positioning System (GPS) trajectory data from the Capital Bikeshare system. A Path Size Logit model is estimated using a hybrid choice set consisting of observed routes and corresponding shortest paths, integrating Geographic Information System (GIS)-based infrastructure variables with computer vision-derived street-level visual features extracted from Street View images (SVI). The results indicate that e-bike riders tend to choose routes that minimize conflicts with both motor vehicles and pedestrians while maintaining travel continuity. Roadway hierarchy substantially moderates the influence of bicycle facilities, with the presence of bicycle facilities having a much greater impact on route choice along major roads than along minor roads. Longer trips also exhibit stronger preferences for cycling infrastructure. Incorporating street-level visual features improves model performance, although their effects are generally smaller than those of road infrastructure, with trees being the only greenery component showing a consistently positive effect. Standardized effect sizes further identify the most behaviorally important route attributes. These findings provide practical evidence for cycling infrastructure planning in the e-bike era.

==> trb_template.tex <==
 % Repository:  https://github.com/chiehrosswang/TRB_LaTeX_tex
%
% Transportation Research Board conference paper template
% version 4.0 Lite (updates made to be compatible in Overleaf and ShareLaTeX)
% 
% 
% When numbered option is activated, lines are numbered.

% \documentclass[numbered]{trbunofficial}
% \usepackage{graphicx}
% \usepackage{makecell}
% \usepackage{tabularx}
% \usepackage{xcolor,graphicx,float}  
% \usepackage{multirow}
% \setlength {\marginparwidth }{2cm}
% \usepackage{todonotes}
% \usepackage{makecell}
% % \usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}
% % For TRB version hide links
% \usepackage[hidelinks]{hyperref}
% \usepackage{colortbl}
% \usepackage{threeparttable}
% % Put here what will go to headers as author
% \AuthorHeaders{Qian, Yin, Scott, and Yan}

% \newcommand{\yiheng}[2][ ]
% {\todo[color=darkblue,inline, #1]{\textcolor{white}{\textbf{Yiheng:} #2}}}
% \newcommand{\yihengshort}[2][ ]
% {\todo[color=darkblue, #1]{\textcolor{white}{\scriptsize\textbf{5:} #2}}}


%\title{Understanding E-Bike Route Preferences: Infrastructure, Streetscape, and Urban Spatial Variation}

\title{Modeling E-Bike Route Choice with Street-Level Imagery and Infrastructure Attributes: A Path Size Logit Analysis in Washington, DC}

%Integrating Street-Level Imagery into E-Bike Route Choice Modeling: A a Path Size Logit Approach in Washington, DC"

% TODO: add macros for easier formatting of \author.
\author{%
  \textbf{Yiheng Qian}\\
  Department of Civil and Coastal Engineering, University of Florida, 1949 Stadium Rd, Gainesville, FL 32611\\
  yihengqian@ufl.edu\\
   \hfill\break%
  \textbf{Zehui Yin}\\
  TransLAB (Transportation Research Lab), School of Earth, Environment \& Society, McMaster University, 1280 Main Street West, Hamilton, ON L8S 4K1\\
  yinz39@mcmaster.ca\\
  \hfill\break% this is a way to add line numbering on empty line
  \textbf{Darren M. Scott}\\
  TransLAB (Transportation Research Lab), School of Earth, Environment \& Society, McMaster University, 1280 Main Street West, Hamilton, ON L8S 4K1\\
  scottdm@mcmaster.ca\\  
  \hfill\break% this is a way to add line numbering on empty line
  \textbf{Xiang Yan}\\
  Department of Civil and Coastal Engineering, University of Florida, 1949 Stadium Rd, Gainesville, FL 32611\\
  xiangyan@ufl.edu\\
  \hfill\break
}


% If words are counted manually, put that number here. This does not include
% figures and tables. This can also be used to avoid problems with texcount
% program i.e. if one does not have it installed.
% \TotalWords{200}

\begin{document}
\maketitle
\section{Abstract}
%This study examines electric-bike (e-bike) route choice behavior in Washington DC using a Path Size Logit model estimated with Global Positioning System data from shared e-bikes. The analysis evaluates how route selection is associated with both detailed cycling infrastructure characteristics and street level micro-built environment features derived from Street View imagery. The results indicate that protected bike lanes are strongly associated with increased route attractiveness, whereas shared and painted lanes tend to deter route choice, particularly on major roads. Residential streets and low stress riding environments are also positively associated with e-bike routing decisions, underscoring the importance of safety, comfort, and cycling network continuity. In addition to infrastructure effects, street level visual attributes show systematic associations with route choice, suggesting that sensory and aesthetic characteristics influence how riders evaluate alternative cycling routes. By integrating street level visual information into a Path Size Logit framework, this study provides new empirical evidence on e-bike route choice in a United States urban context and demonstrates the value of combining behavioral modeling with computer vision based micro-built environment measures to support micromobility planning.

This study examines shared electric-bike (e-bike) route choice behavior in Washington, DC using a Path Size Logit model estimated from GPS-based revealed preference data. The analysis evaluates how e-bike route choice is shaped by cycling infrastructure types, roadway characteristics, elevation, and micro-built environment features derived from Street View imagery. Results show that protected bike lanes on both major and minor roads are strongly preferred by e-bike riders, while shared lanes on major roads exhibit a strong deterrent effect. Painted bike lanes have context-dependent effects on e-bike route choice, enhancing route attractiveness on minor roads but diminishing it on major roads. Moreover, sidewalks and residential streets are positively associated with route choice, suggesting that e-bike users prefer low-stress and flexible riding environments. In addition, we found that street-level visual attributes such as sky visibility, walls, and presence of cars are significantly associated with e-bike route choice behavior. This study provides new empirical evidence on e-bike route choice in a United States city context. By incorporating street-level visual features into a Path Size Logit modeling framework, we demonstrate the value of integrating computer vision with traditional behavioral modeling to support micromobility planning.

%show systematic associations with route choice. Features such as sky visibility, walls, and cars are positively associated, suggesting that micro-scale visual cues may reflect riders’ perceptions of openness, legibility, and corridor context. 




\vspace{1em} 
\noindent\textit{Keywords}: E-bike, Route Choice, GPS, Street View Imagery, Path Size Logit
\newpage



\section{Introduction}



Electric-bikes (e-bikes) have emerged as an increasingly important mode of urban transportation, offering a flexible and energy efficient alternative for short and medium distance travel. As cities seek to promote low carbon mobility and reduce reliance on private automobiles, e-bikes are becoming an integral component of urban transport systems \cite{mcqueen2020bike}. Understanding how e-bike users select routes is therefore essential for designing effective cycling infrastructure, improving safety, and enhancing the overall riding experience \cite{dane2019route}. Such knowledge also supports broader planning decisions, including the placement of supporting facilities such as parking and charging infrastructure.

%\cite{lilasathapornkit2025cycling}
%\cite{arning2023review}

%\cite{fishman2016bikes}



Although a growing body of research has examined bicycle route choice, empirical evidence focusing specifically on e-bikes remains limited. Existing studies suggest that e-bike route choices are context-dependent, with reduced sensitivity to facility type \cite{khavarian2024bike, lilasathapornkit2025cycling} but continued benefits from dedicated cycling infrastructure \cite{singh2025analysing, khavarian2024bike}, as well as an emphasis on route comfort and enjoyment \cite{plazier2017cycling}. However, much of this evidence is drawn from European cities with relatively mature cycling environments \cite{fishman2016bikes}, raising questions about its generalizability to United States urban contexts.


Prior studies on e-bike route choice have emphasized different dimensions of behavior, such as aggregated infrastructure indicators, heterogeneity across e-bike types, and variation among user groups \cite{dane2019route, plazier2017cycling, arning2023review, khavarian2024bike, singh2025analysing, chavis2021bikes}. However, relatively few studies have jointly examined detailed facility types together with roadway context across the full urban street network. In practice, protected, painted, and shared bike lanes, off-street cycleways, and local roads differ substantially in perceived safety and comfort—differences that may be particularly salient for e-bike users, who typically operate at higher speeds and interact differently with surrounding traffic. Explicitly distinguishing these facility types is therefore critical for eliciting meaningful behavioral responses to infrastructure design.

%These inconsistencies point to important limitations in how e-bike route choice has been modeled to date. One key limitation concerns the representation of route attributes. 

Another gap lies in the limited consideration of the street level environment beyond the physical network. Most route choice models depend on Geographic Information System (GIS) based infrastructure data, typically derived from OpenStreetMap (OSM) or municipal sources. While these data provide valuable information on network structure, they often fail to capture sensory and aesthetic attributes of the streetscape that shape how routes are experienced. Elements such as greenery, openness, enclosure, and visible traffic influence perceived comfort, safety, and continuity, yet are rarely incorporated into formal route choice models due to the lack of scalable and systematic measurement approaches.

Motivated by these gaps, this study examines e-bike route choice behavior in DC and surrounding areas using Global Positioning System (GPS) trajectory data from shared e-bikes provided by Lyft. A Path Size Logit (PSL) model is employed to identify key factors influencing route selection. To better capture how riders experience the street environment, the analysis integrates traditional GIS based infrastructure variables with street level visual attributes extracted from Street View imagery. These visual measures allow sensory and aesthetic characteristics of routes to be quantified and incorporated directly into the modeling framework.

This study addresses two central research questions. First, to what extent do different types of road infrastructure, particularly detailed categories of cycling facilities such as protected, painted, and shared lanes, influence e-bike route choice behavior in a United States urban setting. Second, how do micro scale streetscape attributes related to greenery, visibility, enclosure, and traffic conditions shape e-bike route selection. By combining fine grained infrastructure classification with street level environmental information, this study contributes new empirical evidence on how e-bike users evaluate routes in United States cities and demonstrates the value of integrating sensory and aesthetic attributes into behavioral route choice modeling.


\section{Literature review}

Route choice is an individual process within the trip assignment phase of the four-step travel demand model. Route choice modeling plays a pivotal role in understanding the decision-making process of travelers within urban environments. Since studies specifically focusing on e-bike route choice remain limited, our literature review draws on findings from related micromobility modes, including traditional bicycles and electric-scooters (e-scooters). The following subsections introduce commonly used modeling techniques and summarize key factors influencing micromobility route choice as identified in the literature.

\subsection{Route choice modeling approaches}

Various techniques have been employed to analyze and predict route preferences. Depending on data sources, existing studies generally rely on either stated preference or revealed preference approaches. For studies based on survey or interview data, stated preference modeling is commonly adopted \cite{khavarian2024bike}. In contrast, when observed trajectory data are available, route choice behavior is most often analyzed using discrete choice models derived from the random utility maximization framework. In such revealed preference–based studies, the typical workflow involves extracting individual trips from observed data (e.g., GPS trajectories), map-matching these trips to a road network, generating feasible choice sets, computing relevant route attributes, and finally specifying and estimating the route choice model.

Route-based methods are the most common in route choice statistical modeling. These models estimate parameters by comparing observed routes with non-chosen alternatives, each characterized by attributes such as distance, number of junctions, and scenery. Random utility models describe individual choice behavior by assigning a utility to each alternative, composed of observed and random components. The Multinomial Logit (MNL) model is a common example but assumes independence among alternatives. To address this, correction models adjust the utility to capture correlations between similar choices. The most prevalent type is the Multinominal correction model, which adds a correction term to the utility function to account for correlation effects. A typical example is the PSL model, which has a long theoretical history. This model extends the Multinomial Logit by including a Path Size factor in the utility function, penalizing overlapping routes within the choice set (i.e., trips sharing one or more segments). PSL has been widely used to handle route choice problems \cite{ton2018evaluating,marra2020determining,nielsen2021relevance,yap2021taking,sevtsuk2021big,meister2023route}.

This PSL approach depends on generating a choice set that includes unchosen alternatives, which itself is a distinct research area. The most used measure to evaluate the quality of choice sets is the ability to reproduce the observed behavior. \citet{ton2018evaluating} identifies breadth-first search on link elimination as the most effective method for generating a choice set. However, in large and fragmented urban networks, concerns over reproducibility and computational burden remain.



\subsection{Factors influencing route choice of micromobility}


Although e-bikes and bicycles share operational and spatial similarities, research on bicycle route choice is far more extensive and can provide a useful foundation for modeling e-bike behavior. A well established body of literature on cycling highlights consistent preferences for shorter routes with dedicated infrastructure, scenic surroundings, and minimal interaction with traffic, intersections, and steep slopes. For example, \citet{meister2024comparative} summarized that cyclists tend to avoid routes with high gradients, mixed traffic, and traffic signals. Similarly, \citet{lukawska2023joint} found that cyclists prefer green or waterfront environments, and protected lanes, with stronger preferences among infrequent riders and long trips. \citet{fosgerau2023bikeability} further quantified generalized costs across infrastructure types, emphasizing the value of protected lanes, especially on major roads, and the attractiveness of cycleways in green or industrial zones due to their traffic separation.

%\citet{zhang2021type} conducted a pioneering study using campus-based trip data, showing a strong preference for bikeways and avoidance of stairs, with e-scooter users willing to travel significantly longer distances to avoid barriers. However, such campus-specific findings may not generalize to complex urban settings. 


At the same time, e-bikes exhibit distinct behavioral patterns. As summarized in the literature \cite{hallberg2021modelling}, electric bicycle users tend to travel at higher speeds and also cover longer distances or travel for longer durations. Taken together, these findings suggest that increased speed is not used solely to save travel time, but also enables different types of trips. Moreover, although e-bikes offer enhanced speed, this speed advantage may vary across roadway contexts and facility types \cite{langford2015risky}. These characteristics indicate that findings from traditional cycling studies may not fully translate to e-bike contexts and highlight the need for dedicated investigation.


A growing body of research has examined route choice behavior among traditional bicycle users, yet empirical evidence focusing specifically on e-bike riders remains limited. Existing studies on e-bike route preferences report context-dependent and heterogeneous findings. One study in Dublin, Ireland, emphasizes the importance of safe and uninterrupted cycling space, highlighting the role of protected infrastructure in encouraging e-bike use \cite{singh2025analysing}. Meanwhile, a study conducted in Helsinki, Finland, indicates that e-bike users are relatively less sensitive to facility type and road classification, although dedicated cycling routes remain beneficial \cite{khavarian2024bike}; no statistically significant preference for protected infrastructure is observed among e-bike riders in Melbourne, Australia \cite{lilasathapornkit2025cycling}. Beyond this, an interview study conducted in Groningen, the Netherlands, found that e-bike users generally preferred enjoyable and quiet routes except when time constraints or adverse weather conditions were present \cite{plazier2017cycling}. Much of this literature is based on European cities with relatively mature cycling cultures and infrastructure \cite{fishman2016bikes}. Consequently, the extent to which these findings generalize to United States urban contexts remains uncertain.

These discrepancies point to gaps in the current literature, particularly the lack of nuanced modeling that incorporates both streetscape perception and detailed infrastructure classification. This study addresses these gaps by focusing on Washington, DC, an urban environment with diverse spatial contexts. Using revealed preference data from shared e-bike trips, we model route choice behaviors across different city zones. Our approach integrates traditional GIS data with Street View derived visual features, enabling a richer understanding of how both physical infrastructure and perceptual elements influence e-bike route preferences. By applying consistent methodology in a complex real world setting, our study contributes to more generalizable insights that support infrastructure design and urban mobility planning.
 
\section{Data}
\subsection{E-bike trip trajectories}

This study focuses on Washington, DC, where bikesharing was first introduced through SmartBike DC in 2008, followed by the launch of Capital Bikeshare in 2010. Electric-assist bicycles were subsequently introduced through a pilot deployment within the Capital Bikeshare system in 2018 \citep{DC_CaBi_Ebike_2018}. Capital Bikeshare is now operated by Lyft. We utilize GPS trajectory data from shared e-bikes provided by Lyft, covering the entire calendar year of 2023. The dataset corresponds to the Capital Bikeshare service area, which includes not only the District of Columbia but also surrounding jurisdictions such as Arlington, VA. For simplicity, we refer to this broader service area as ``DC'' throughout the remainder of the text. Each entry in the dataset represents a GPS point, including latitude, longitude, a timestamp, and a unique e-bike ID that remains stable over time. This consistent ID allows us to accurately reconstruct individual e-bike trajectories. To ensure data quality, We then refined the trip data by excluding trips shorter than 2 minutes, longer than 90 minutes, or distances outside 0.4--3 miles. After processing, 65,521 valid trips were identified for this study, which incorporate all trip trajectories in DC.

This cleaned and structured trip dataset forms the basis for our subsequent modeling of e-bike route choice behavior. To enable this, we implemented a three-step methodological framework: 1) preparing the road network and applying a map matching algorithm to align raw GPS trajectories with the transport infrastructure; 2) cleaning and refining matched trajectories to ensure valid origin-destination (OD) pairs; and 3) constructing behaviorally plausible choice sets for route choice modeling. These steps ensure that the input data are spatially accurate and behaviorally meaningful for subsequent model estimation.

\subsection{Map matching}

Map matching is a crucial step that assigns GPS-based trajectories to a series of links or nodes (and related network attributes) to precisely reconstruct users' actual paths. As reviewed in a recent study by \citet{berjisian2023evaluation}, map matching for active travel modes is more complex than for car travel, highlighting two main challenges:
1) Cyclists and pedestrians do not always stick to official roads and paths, sometimes opting for shortcuts that may be missing from the network.
2) The types of infrastructure these users are allowed to use, and actually do use, are not always clearly defined. Individuals often switch between closely parallel facilities that traditional matching algorithms struggle to detect.

We utilized the Python package Leuven.MapMatching \cite{meert2018hmm} to map-match the trip GPS trajectories based on a Hidden Markov Model with non-emitting states \cite{newson2009hidden}. The map-matching was conducted on the OSM walking road network \cite{OpenStreetMap}, with one-way street restrictions removed to better reflect the fewer constraints typically faced by cyclists compared to drivers. To enhance matching accuracy, we applied a series of custom preprocessing steps, including the removal of GPS outliers and dwelling points. Additionally, turn events were extracted during the map-matching process by analyzing changes in road segment bearings. Specifically, bearing changes between 75° and 170° were classified as right turns, between 170° and 190° as U-turns, and between 190° and 285° as left turns. This map-matching process was first introduced and utilized in \citep{yin2026decoding}.

Using the selected valid trip trajectories and the OSM walking road network \cite{OpenStreetMap}, we applied customized map-matching, assigning each trip a unique ID. The output included the trip ID, the sequence of traversed links and nodes, their corresponding geometries matched to the road network, and the counts of left, right, and U-turns. We manually verified a subset of randomly sampled routes by comparing the map-matched paths to the original GPS trajectories. This examination revealed no significant issues, indicating the robustness of the used approach.

To prepare inputs for the choice set generation, we conducted post-processing on the map-matching results. Trips containing duplicate nodes or links within a single trajectory, such as circular routes or back-and-forth movements, were excluded. These patterns often indicate non-purposeful or leisure travel rather than trips between distinct locations. In many such cases, the origin and destination are very close, resulting in unrealistically short alternative routes that do not reflect the user's actual decision-making. Including these trips could compromise the validity of route choice modeling. The generation of the choice set in this study is grounded in revealed behavior, rather than synthetic route enumeration. Specifically, we grouped trips with identical OD pairs into a shared choice set. To account for minor locational discrepancies in GPS points, we further allowed spatial tolerance by treating OD pairs as equivalent if both their origins and destinations fell within a 50-meter radius of each other. This spatial clustering enabled us to consolidate trips with near identical spatial intentions into unified OD groups. For each OD group, all unique routes observed from the trip data were extracted, and their corresponding frequencies (i.e., how many users chose each route) were calculated. To ensure modeling reliability, we retained only those OD groups that satisfied two criteria:
\begin{enumerate}
    \item The group included at least three distinct routes, forming a meaningful choice set.
    \item The most frequently chosen route within the set had been selected by at least two users, ensuring that noise is limited.
\end{enumerate}

This behavior based choice set construction approach has several advantages. First, it ensures realistic and behaviorally valid alternatives, as all candidate routes are derived from actual observed choices. Second, it avoids reliance on algorithmically generated paths that may not reflect users' real world preferences, constraints, or awareness. Third, by incorporating route frequency, it allows for modeling that reflects the relative attractiveness of each alternative under naturalistic conditions.

%To further explore spatial heterogeneity in route preferences, we defined a central area by creating a 3-kilometer radius buffer centered on the White House, the symbolic and geographic core of Washington, DC. This buffer was constructed using the White House's geographic coordinates (38.8977° N, 77.0365° W) as the center point. All route segments (links) and trips were then spatially intersected with this buffer to classify whether they fell entirely inside or outside the central area. This spatial segmentation enables us to compare user preferences and route choice behavior across distinct urban contexts, namely, the dense urban core versus the more peripheral areas. 


Our filtered dataset includes 1,285 OD pairs (with 5 alternatives in average), with 677 classified as outside and 608 as inside the central buffer area. This split provides a relatively balanced spatial distribution of trip origins and destinations, allowing for meaningful comparisons between central and peripheral urban environments.




\subsection{Street View images}




To capture the visual and perceptual qualities of the riding environment, we extracted streetscape features from Street View imagery using computer vision. A total of 54,601 images were sampled and collected from an online third-party provider at unique geographic locations along the candidate network. Each image was processed using SegFormer \cite{DBLP:journals/corr/abs-2105-15203}, a transformer-based semantic segmentation model pre-trained on ImageNet and fine-tuned on ADE20K. The output assigns pixel-level labels across various categories, including natural elements (e.g., tree, sky, grass) and built environment features (e.g., building, wall, traffic light).

To represent these visual elements at the route level, we adopted two types of metrics depending on the spatial characteristics of the features. For large-scale, spatially continuous elements like trees, buildings, or sky, we computed the average pixel proportion across all images along each route. This captures their general visual dominance and environmental continuity. This approach allows us to incorporate both physical and perceptual dimensions of the environment into the route choice model, offering a more complete view of how streetscape features shape micromobility behavior.


%For small, discrete elements such as traffic lights, we relied on buffer-based object counts along the route, which better reflect their functional presence than pixel-based measures, given their low visibility in individual images. 

\section{Route choice model}
This section outlines the methodology used to model e-bike route choice behavior. We begin by detailing the variables used in the model, then we introduce the PSL model, which accounts for overlapping routes and is well suited for analyzing route choice behavior. 



\subsection{Variables affecting e-bike route choice}

To identify the factors that may influence e-bike users' route choices, we generated attributes for all routes within the choice set. We have considered four categories of variables: trip characteristics, elevation, road type and infrastructure, and micro-built environment features derived from Street View images, Table \ref{var} provides detailed information about these variables. 

\begin{table}
\centering
\caption{Variables in the e-bike route choice model}\label{var}
\vspace{4pt} 
\small 
\renewcommand\cellalign{tl}  
\renewcommand\arraystretch{1.1} 
\resizebox{\textwidth}{!}{
\begin{tabular}{lll}
\hline
\textbf{Variable} & \textbf{Description} &  \\
\hline
\textbf{Trip attributes} &  &  \\
Length & Total length of all links in the route (mile) &  \\
Turns & Total number of left and right turns per mile of route &  \\
Traffic lights & Traffic light counts per mile of route &  \\
\hline
\textbf{Road type and infrastructure} &  &  \\
Major  & \begin{tabular}[c]{@{}l@{}}OSM tag:   highway=\{``primary'',``secondary'',``tertiary'',``unclassified''\}   that have \\ at least two car lanes in at least one direction\end{tabular} &  \\
Major with shared & \begin{tabular}[c]{@{}l@{}}Length of major roads with   shared bike markings (mile)\\      OSM tag:      cycleway=\{``shared\_lane'', ``share\_busway''\}\end{tabular} &  \\
Major with painted & \begin{tabular}[c]{@{}l@{}}Length of major roads with   painted bike lanes (mile)\\      OSM tag:      cycleway=\{``lane'', ``opposite\_lane''\}\end{tabular} &  \\
Major with protected & \begin{tabular}[c]{@{}l@{}}Length of major roads with protected bike lanes (mile)\\      OSM tag:     cycleway=\{``track'', ``separate''\}\end{tabular} &  \\
Minor  & \begin{tabular}[c]{@{}l@{}}OSM tag:   highway=\{``primary'',``secondary'',``tertiary'',``unclassified''\}   that have \\ at most one car lane per direction\end{tabular} &  \\
Minor with shared & \begin{tabular}[c]{@{}l@{}}Length of minor roads with   shared bike markings (mile)\\      OSM tag:   cycleway=\{``shared\_lane'', ``share\_busway''\}\end{tabular} &  \\
Minor with painted & \begin{tabular}[c]{@{}l@{}}Length of minor roads with   painted bike lanes (mile)\\      OSM tag:  cycleway=\{``lane'',   ``opposite\_lane''\}\end{tabular} &  \\
Minor with protected & \begin{tabular}[c]{@{}l@{}}Length of minor roads with   protected bike lanes (mile)\\      OSM tag:   cycleway=\{``track'',   ``separate''\}\end{tabular} &  \\
Residential roads & \begin{tabular}[c]{@{}l@{}}Length of residential roads   (mile)\\      OSM tag: highway=``residential''\end{tabular} &  \\
Bikeable sidewalks & \begin{tabular}[c]{@{}l@{}}Length of designated bikeable   sidewalks (mile)\\       OSM tag:   highway=``footway'', bicycle=``yes''\end{tabular} &  \\
Off-street cycleways & \begin{tabular}[c]{@{}l@{}}Length of off-street cycleways   (mile)\\       OSM tag:   highway=``cycleway''\end{tabular} &  \\
Stairs & \begin{tabular}[c]{@{}l@{}}Length of  flights of steps (mile)\\       OSM tag: highway=``steps''\end{tabular} &  \\
Pedestrian zones & \begin{tabular}[c]{@{}l@{}}Length of roads used mainly for   pedestrians (mile)\\       OSM tag:   highway=``pedestrian''\end{tabular} &  \\
Shared paths & \begin{tabular}[c]{@{}l@{}}Length of shared paths between   cyclists and pedestrians (mile)\\      OSM tag: highway=\{``path'',``service''\}\end{tabular} &  \\
\hline
\textbf{Elevation} &  &  \\
Slope 2\%--6\% & Length of links with 2\%--6\% positive slope (mile) &  \\
Slope 6\%--10\% & Length of links with 6\%--10\% positive slope (mile) &  \\
Slope over 10\% & Length of links with slope greater than 10\% (mile) &  \\
\hline
\textbf{Micro-built environment features} &  &  \\
Tree & Average of tree pixels proportion from Street View points along the route &  \\
Plant & Average of plant pixels proportion from Street View points along the route &  \\
Grass & Average of grass pixels proportion from Street View points along the route &  \\
Sky & Average of sky pixels proportion from Street View points along the route &  \\
Walls & Average of wall pixels proportion from Street View points along the route &  \\
Cars & Average of car pixels proportion from Street View points along the route &  \\

\hline
Path size & Path size term to account for route overlapping & \\
\hline
\end{tabular}
}
\end{table}


The variable ``Turns'' captures both left and right turns along the route, calculated during the map-matching procedure. While a potential extension could involve separating left and right turns, we observed a high correlation between the two, so we retained a combined variable to avoid multicollinearity.

All road type and elevation variables were measured in miles. The classification of road type and cycling infrastructure follows previous studies \cite{fosgerau2023bikeability,lukawska2023joint}, and we further refined the infrastructure categories in the context of e-bike travel. Specifically, we relied on OSM data, using the highway and cycleway tags to define road types and infrastructure combinations, as detailed in Table \ref{var}. Elevation attributes were derived from 2' contour elevation data available via Open Data DC \cite{DCGIS_ElevationPoints_1999}. For each segment, slope was estimated by taking the elevation difference between its origin and destination points, divided by the segment length. Informed by prior literature \cite{meister2023route}, slopes were then categorized into three groups: 2\%–-6\%, 6\%–-10\%, and greater than 10\%. For the micro-built environment variables, we constructed a 25-meter buffer around each Street View point and identified intersecting trip trajectories to calculate the average feature values along each route. 

%Given the segmentation errors inherent in Street View-based computer vision models, low confidence values were excluded from the aggregation to improve the reliability of environmental perception measures.

In the OSM road network, ``footway'' typically does not appear as tags on main roads but rather exist as independent paths running parallel to them. Due to inherent GPS inaccuracies and the possibility that users are riding on bike lanes or sidewalks adjacent to main roads, it is often difficult to determine with certainty whether a user is truly riding on a sidewalk. This can lead to alignment mismatches during the matching process. To mitigate this issue, we incorporated the bicycle=``yes'' tag from OSM to identify bikeable sidewalks, thereby improving the interpretability of this feature in the model.

Another potential source of confusion is the cycleway tag. In OSM, highway=``cycleway'' typically refers to a separate cycleway, not an inherent part of the main road, particularly not on-road cycle lanes. To clarify this distinction, we label these segments as off-street cycleways, which better reflects their nature as physically separated cycling infrastructure.


\subsection{Path size logit model}

The MNL model is a method used to model the relationship between a multilevel dependent variable and a set of independent variables \cite{ben1985discrete}. In other words, given a set of explanatory variables, the MNL model can predict the probability of alternative outcomes for a multimodal response variable. However, MNL is unsuitable for route choice modeling with overlapping routes because it assumes that cyclists perceive each route as an independent alternative \cite{bekhor2006evaluation, prato2009route}. To account for overlapping routes, the PSL model incorporates a correction factor (the path size term) into the route utility within the MNL framework. Thus, the PSL model is appropriate for studying factors influencing route choice behavior and is the most commonly used model in bicycle route choice research \cite{halldorsdottir2014efficiency,meister2024comparative,lukawska2023joint,meister2023route,ton2018evaluating,scott2021route}.


To calculate the path size term (\(PS_i\)) for route \(i\), we use the following formula:
\begin{equation}
    PS_i = \sum_{a \in i} \frac{L_a}{L_i} \frac{1}{\sum_{j \in C} \delta_{aj}}
\end{equation}
where \(L_a\) is the length of road link \(a\), \(L_i\) is the length of route \(i\), \(\delta_{aj}\) is an indicator function that equals 1 if road link \(a\) is in route \(j\) and 0 otherwise, and \(C\) is the choice set of all routes.

% Path Size Logit Model Utility
The latent deterministic utility (\(V_i\)) for route \(i\) in the PSL model is given by:
\begin{equation}
    V_i = \beta X_i + \ln(PS_i)
\end{equation}
where \(\beta\) is a vector of generic coefficients, \(X_i\) is a vector of observed attributes for route \(i\), and \(PS_i\) is the path size term for route \(i\).

% Probability of Choosing Route i
The probability (\(P_i\)) of choosing route \(i\) is then given by the standard multinomial logit formulation:
\begin{equation}
    P_i = \frac{e^{V_i}}{\sum_{j \in C} e^{V_j}}
\end{equation}


These equations together form the basis of the PSL model, which accounts for route overlap by incorporating the path size term into the utility calculation, thereby providing a more robust representation of route choice behavior.
\begin{figure}[H]
  \centering
  \includegraphics[width=0.7\textwidth]{roadinfra.jpg}
  \caption{Illustration of roadway characterization and bicycle facility types: 
  (1) major roads, 
  (2) minor roads, 
  (3) protected lanes, 
  (4) painted lanes, 
  (5) shared lanes.
  Source: OpenStreetMap (OSM), Google street view, District Department of Transportation (DDOT).}
  \label{var1}
\end{figure}

\section{Results}


We used the R package \texttt{clogit} \cite{reid2014clogitL1} to estimate the e-bike route choice model using maximum likelihood. 
Table \ref{model} reports the estimated coefficients, with statistical significance indicated for each variable. 
The C-index, ranging from 0 to 1, measures a model's ability to correctly rank the chosen route relative to non-chosen alternatives, with values above 0.5 indicating performance better than random choice. 
The C-index of 0.813 indicates strong predictive performance in distinguishing chosen routes from alternative options. 
Overall, the results suggest that the model captures key factors underlying users' route choice behavior.

%/0.825/0.884
We found that the probability of choosing a route is negatively and significantly correlated with route length, indicating that e-bike users tend to prefer shorter routes when other variables are held constant. 
This finding is consistent with most existing bike and e-bike route choice studies, which also report a negative association between route length and utility \cite{halldorsdottir2014efficiency,meister2024comparative,lukawska2023joint,meister2023route,ton2018evaluating,scott2021route}. 
Additionally, the number of turns is significantly negatively associated with route choice, suggesting that e-bike users generally avoid routes with frequent directional changes. 
Traffic lights also exhibit a significant negative effect, indicating that signalized intersections are generally perceived as impediments in e-bike route selection.




\begin{table}[H]
\centering
\normalsize
\renewcommand\arraystretch{1.5}	
\caption{E-bike route choice model}\label{model}
\vspace{4pt} 
\resizebox{0.8\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{lllll}
\hline
\textbf{Variable} & Estimated Coefficient & Standard Error & $z$-statistic & Significance Level \\
\hline
Length & -13.51 & 2.27 & -5.95 & *** \\
Turns & -0.26 & 0.02 & -11.71 & *** \\
Major  & -4.73 & 1.47 & -3.22 & ** \\
Major with shared & -22.38 & 7.78 & -2.88 & ** \\
Major with painted & -19.78 & 5.60 & -3.53 & *** \\
Major with protected & 17.33 & 4.17 & 4.16 & *** \\
Minor  & -2.61 & 2.57 & -1.02 &  \\
Minor with shared & -5.47 & 3.53 & -1.55 &  \\
Minor with painted & 6.89 & 1.73 & 3.98 & *** \\
Minor with protected & 17.18 & 6.03 & 2.85 & ** \\
Residential roads & 3.55 & 1.66 & 2.14 & * \\
Bikeable sidewalks & 19.41 & 4.86 & 3.91 & *** \\
Off-street cycleways & -4.18 & 1.84 & -2.27 & * \\
Stairs & -624.67 & 518.48 & -1.20 &  \\
Pedestrian zones & 6.60 & 14.31 & 0.46 &  \\
Shared paths & -5.58 & 3.68 & -1.52 &  \\
Slope 2\%--6\% & 1.26 & 2.14 & 0.59 &  \\
Slope 6\%--10\% & 2.70 & 4.18 & 0.65 &  \\
Slope over 10\% & -18.43 & 5.09 & -3.62 & *** \\
Tree & 0.05 & 0.09 & 0.62 &  \\
Plant & -0.04 & 0.14 & -0.28 &  \\
Grass & -0.27 & 0.09 & -3.07 & ** \\
Sky & 0.25 & 0.11 & 2.23 & * \\
Walls & 0.49 & 0.11 & 4.53 & *** \\
Cars & 0.45 & 0.14 & 3.33 & *** \\
Traffic lights & -0.28 & 0.08 & -3.55 & *** \\
Path size & -0.28 & 0.08 & -3.55 & *** \\
\hline
C-index & \multicolumn{4}{c}{0.813} \\
Sample size & \multicolumn{4}{c}{1285} \\
\hline
\end{tabular}
\par\vspace{2mm}
\small\textbf{Note:} *** p $<$ 0.001, ** p $<$ 0.01, * p $<$ 0.05, . p $<$ 0.1
\end{threeparttable}}
\end{table}







Major roads exhibit an overall negative effect on route choice. Specifically, major roads equipped with shared or painted bike lanes significantly reduce the probability of a route being chosen, with shared lanes showing a more pronounced negative impact. In contrast, major roads with protected bike lanes are significantly preferred by e-bike users. This pattern suggests that riders are sensitive to the type of cycling infrastructure provided and adjust their route choices accordingly. This pattern reinforces earlier findings from the literature. For instance, \cite{monsere2014lessons} showed that the installation of protected bike lanes led to increased cycling activity and caused 24\% of users to shift from other routes. Similarly, \cite{mcneil2015influence} found that while painted buffers offer some comfort, even minimal physical protection provides higher perceived comfort and safety. 




 
%explain may be cautious
%\cite{chavis2021bikes}
%some literature find e-bike usage increase;



Minor roads show no significant overall effect on route choice, and minor roads with shared lanes also do not exhibit a significant impact. These estimated coefficients suggest that minor roads are generally perceived as more acceptable riding environments relative to major roads, offering a neutral riding environment. Both painted and protected lanes on minor roads are associated with positive effects, with protected lanes demonstrating a stronger influence consistent with the patterns observed for major roads. Similarly, residential roads show a significant positive effect, indicating that low-traffic neighborhood streets are broadly preferred by e-bike users. Taken together, these results suggest that appropriate infrastructure enhancements on major and minor roads may have the potential to improve their attractiveness for e-bike travel.


%In the outside model, which represents urban fringe areas, major roads show no significant overall effect, indicating that cyclists do not have a consistent preference for or against major roads in suburban environments. However, the differences among types of cycling infrastructure are more pronounced. As in the general model, protected lanes significantly increase the probability of route choice, while shared and painted lanes significantly reduce it. Notably, the negative effects of shared and painted lanes are even stronger in the outside model, suggesting that the higher vehicle speeds and more exposed traffic environments in suburban areas intensify cyclists’ perceived risks, making non-separated infrastructure less acceptable. This result further underscores the critical importance of high-quality, physically separated cycling infrastructure in suburban settings. Meanwhile, minor roads in the outside model exhibit a generally positive influence, and minor roads with various types of cycling infrastructure also show positive effects. In particular, minor roads with protected lanes significantly increase the likelihood of being chosen. This suggests that, in suburban areas, minor roads are relatively preferred by e-bike users. Compared to major roads, minor roads tend to have moderate traffic flow and lower traffic pressure, while still offering better accessibility and connectivity than other road types. Similarly, residential roads have a significant positive effect, reinforcing the appeal of low-stress, local street networks in suburban environments. Overall, the outside model, compared to the general model, reveals stronger preferences for minor roads and a clearer endorsement of separated infrastructure in enhancing route attractiveness.

%In the inside model, which represents central urban areas, all major road variables have negative coefficients, with only general major roads reaching statistical significance. This indicates that cyclists tend to avoid major roads in general, but show lower sensitivity to the specific types of infrastructure they contain. This may be attributed to the dense street networks and abundant alternative paths in city centers, where cyclists are more inclined to choose smaller, low-stress routes, thereby reducing reliance on and perception of differences among infrastructure types on major roads. Additionally, the prevalence of traffic control and calming measures in urban cores may further diminish the marginal safety impact of different facility types. Similarly, minor roads also show overall negative effects in the inside model. Minor roads with shared lanes significantly reduce the probability of route choice, and even protected minor roads fail to exhibit a positive effect (the coefficient is negative, though not significant). In this context, residential roads also have a negative but insignificant effect, contrasting with their positive roles in other areas. This contrasts with the results from the general and outside models, suggesting that in dense city environments, the road type and perceived traffic pressure may outweigh the influence of specific infrastructure characteristics. Taken together, the inside model suggests that in central urban areas, e-bike users are more likely to avoid major roads regardless of infrastructure quality. This highlights the importance of reducing traffic pressure and improving micro-environments over simply upgrading infrastructure when aiming to enhance the attractiveness of cycling in dense urban settings.

As previously noted, the sidewalks analyzed in this study refer exclusively to pedestrian paths explicitly tagged with bicycle=``yes'' in OSM data, indicating that bicycle access is legally permitted, while cycleways refer to off-street cycling facilities that are physically separated from motor vehicle lanes and do not include on-road features such as painted or shared lanes. The estimation results show that bikeable sidewalks are positively and significantly associated with route choice, whereas off-street cycleways exhibit a significant negative effect. This suggests that, within the observed travel context, bikeable sidewalks may provide relatively low-stress alternatives to on-road facilities, particularly in environments characterized by constrained space or heavy traffic. In contrast, the negative association observed for off-street cycleways may reflect network-related limitations such as fragmented layouts, indirect routing, or reduced network continuity, which can reduce their attractiveness for utilitarian e-bike trips. Given that the analysis focuses on shared e-bike users and excludes trips with circular or back‑and‑forth movements, thereby emphasizing utilitarian travel that prioritize travel efficiency and directness, such characteristics may disproportionately discourage the use of off-street facilities. More broadly, these results point to a context-dependent role of cycling infrastructure, underscoring that the effectiveness of different facility types may vary with urban spatial structure, network design, and cycling trip purposes.

The model results indicate that slope significantly influences e-bike route choice. In particular, routes containing segments with slopes exceeding 10\% are significantly less likely to be chosen, indicating a strong aversion to steep inclines among e-bike users. In contrast, moderate slopes show weaker and not significant effects, suggesting that only substantial elevation changes systematically deter route selection. This pattern implies that while electric assistance reduces the need to avoid all uphill segments, users remain skeptical to steep gradients that may impose physical effort, reduce comfort, elevate injury risk, or affect travel efficiency. Similar deterrent effects of steep terrain have also been documented in the micromobility literature, including \citep{broach2012cyclists} and \citep{yin2026pedal}. In addition to slope-related deterrents, physical barriers are also examined. Stairs show a negative but statistically non-significant association with route choice.


%Finally, we analyzed the effects of different types of greenery-related POIs, and found that their influence varies significantly by vegetation type and spatial context. In suburban areas, trees exhibit a significant positive effect, potentially reflecting their role as spatial indicators of pleasant riding environments such as tree-lined avenues or green corridors. In contrast, the effect of trees is close to negative in city centers, possibly because they are often located in areas with constrained space and complex traffic, which may reduce route attractiveness. Plant-related greenery is not significant in any model, suggesting that low-lying vegetation—due to limited visibility and insufficient shading—does not offer clear behavioral cues or enhanced comfort for riders. Grass shows a significant negative effect in both the general and outside models, likely because it is commonly found near open spaces, parks, or plazas, which tend to have lower connectivity with the cycling network and may introduce spatial discontinuities. This negative association is especially evident in peripheral areas, where high proportions of grass may signal a “non-primary path,” leading to avoidance behavior. Overall, the influence of greenery on e-bike route choice appears to be driven less by visual aesthetics and more by its functional value and its role as an implicit indicator of route continuity and riding comfort.

Finally, we examine the effects of different types of greenery and visual elements derived from street-level imagery and find that their influence on e-bike route choice varies by feature type. Trees and plants do not exhibit statistically significant effects on route choice. Grass, in contrast, is negatively and significantly associated with route choice, potentially reflecting its frequent presence in parks, plazas, or open spaces that are less integrated into the cycling network or involve indirect routing. Taken together, these findings suggest that greenery-related features influence route choice primarily when they are systematically linked to network structure rather than aesthetic presence alone. Sky visibility, the presence of cars, and walls are positively and significantly associated with route choice. Sky visibility may signal openness and navigability, while visible traffic can convey information about route activity and accessibility. The positive association for walls likely reflects the presence of continuous built edges or physical separation along the street, which may enhance enclosure, legibility, or perceived protection. Overall, these street-level visual cues or micro-built environment features appear to function less as purely aesthetic elements and more as indicators of spatial organization and continuity that shape how e-bike users evaluate comfort and traffic stress along alternative routes.


%Trees and plant does not exhibit a significant effect, likely due to its limited visual prominence and functional relevance at the street level. Grass, in contrast, is negatively associated with route choice, potentially reflecting its frequent presence in parks, plazas, or open spaces that are less integrated into the cycling network or involve indirect routing. These findings suggest that greenery affects route choice less through aesthetic appeal alone and more through its role as an implicit indicator of network continuity, comfort, or potential barriers. Consistent with this interpretation, other visual elements also exhibit systematic associations with route choice. Sky visibility and the presence of cars show significant effects, indicating that open views and visible traffic can convey information about route accessibility, exposure, or traffic conditions, which e-bike users appear to factor into their decisions. Walls are positively associated with route choice, suggesting that continuous built edges may enhance enclosure and perceived safety at the street level. Overall, the influence of street-level visual cues or micro-built environment features reflects not only sensory or aesthetic perception but also the spatial and functional meanings these elements convey, shaping how riders interpret comfort, continuity, and traffic stress along alternative routes.

\section{Discussion}

This discussion is organized in two parts. We first highlight broader implications of our findings for understanding e-bike travel behavior and for designing micromobility-friendly infrastructure. We then place our e-bike results in the context of prior evidence for bicycles and e-scooters to identify shared and mode-specific route choice mechanisms. 

%We found that e-bike users' preferences for road types, cycling infrastructure, and micro-built environment features are closely intertwined with broader network structure.

\subsection{Implications for E-bike Route Choice Mechanisms}

%existing literature showing that micromobility usage is negatively correlated with posted speed limits \cite{PBOT2018,zhang2021type}. 

In this section, we compare the effects of road types, cycling infrastructure, and micro-built environment features based on our model results, with the goal of gaining a more detailed understanding of the route choice mechanisms among e-bike riders. This includes examining factors' mutual interactions, identifying potential complementary roles, and analyzing the relative strength and organization of their impacts. Such analysis helps us better investigate how e-bike users currently perceive the riding environment, and provides insights into how to make targeted adjustments and improvements that can expand and enhance the space available for e-bike travel.

While existing studies have consistently demonstrated that protected bike lanes outperform painted or shared facilities in terms of both objective safety and perceived comfort \footnote{Empirical studies demonstrate that protected bike lanes provide substantially greater physical protection compared to painted or shared facilities. The average passing distance between motor vehicles and cyclists is approximately 93cm on roads without bike lanes, 101cm with painted lanes, and 166cm with protected lanes, with the latter virtually eliminating dangerously close passes \cite{nolan2021bicycle}. In terms of perceived safety, survey-based findings similarly indicate that striped or painted buffers offer some comfort improvements \cite{mcneil2015influence}, but protected lanes are associated with significantly higher comfort levels \cite{monsere2014lessons}. Even minimal separation, such as plastic flexposts, has been shown to substantially increase perceived comfort among cyclists with safety concerns \cite{mcneil2015influence}.}, there remains limited discussion on the finer-grained mechanisms through which these facilities function across different road classifications. Building on this, we further discuss how facility types interact with roadway hierarchy and contribute to the observed variation in route choice behavior. 


Painted bike lanes show substantial heterogeneity across different road classifications. Since major roads are typically associated with higher vehicle speeds and traffic volumes, painted lanes may fail to provide a sufficient sense of protection. Specifically, painted lanes on major roads are among the most negative factors in our model, only slightly less deterrent than shared lanes on major roads. In contrast, on minor roads, painted lanes perform much better than shared lanes. Although still weaker than protected facilities, they appear to provide a more acceptable riding environment. One plausible explanation is that the protection offered by painted lanes is inherently ambiguous and less reliable. As a result, riders’ evaluation of painted facilities depends heavily on the surrounding traffic context, leading to strong road type interactions in route choice. In contrast, High-quality physical separation can significantly alleviate the discomfort and perceived risk associated with high-speed, high-traffic environments, making e-bike users more willing to select such routes even on major roads. Besides, once a road is equipped with protected bike lanes, the difference between major and minor roads becomes virtually negligible. The estimated effect values are 17.33 for major roads and 17.18 for minor roads with protected facilities. A deeper implication is that protected bike lanes, at the subjective level or within the riders’ decision-making process, “flatten” or neutralize the influence of road classification on route choice. Such that, in the presence of physical protection, the distinction between major and minor roads disappears to some extent. In contrast, painted bike lanes do not offer this level of psychological compensation so that their effect remains strongly conditioned by the inherent characteristics of the road. This contrast reveals a key mechanism: protected bike lanes not only increase the intrinsic attractiveness of a given path, but also restructure how riders cognitively perceive their riding environment. When making decisions, users focus more on the clearly delineated and physically secured cycling space, rather than on the broader attributes of the road itself. This structural shift in attention and perception is likely an explanation why protected bike lanes are able to mitigate the influence of roadway hierarchy.


%\cite{monsere2014lessons}
%91% of surveyed residents agreed with the statement, "I support separating bikes from cars." This agreement was high among primary users of all modes (driving, walking, transit, and bicycling), though motorists expressed concerns about the impacts of protected lanes on congestion and parking. 

%Most residents also agreed with the statement "I would be more likely to ride a bicycle if motor vehicles and bicycles were physically separated by a barrier," with "Interested but Concerned" residents expressing the highest level of agreement at 85%. Nearly three times as many residents felt that the protected bike lanes had led to an increase in the desirability of living in their neighborhood, as opposed to a decrease in desirability (43% vs 14%).
%These patterns reflect an overarching concern for safety, comfort in environments characterized by higher traffic speeds and limited routing alternatives. 
%low-traffic, flexible riding environments
Besides, among road environment attributes, bikeable sidewalks show the largest positive and statistically significant association, exceeding even that of protected facilities on major/minor roads. A likely mechanism is that when arterial corridors impose high stress and bike lanes are absent or provide insufficient protection, sidewalks can serve as a parallel low-stress substitute that offers perceived safety and comfort. Note that “bikeable sidewalk” does not necessarily imply that bicycle facilities are absent along the corridor. Rather, many DC corridors are characterized by an asymmetric cross-sectional configuration in which high-quality on-street facilities (e.g., protected lanes) exist on one side, while the other side retains wide, continuous sidewalks. In such contexts, sidewalks may be used as a complementary riding option with more flexibility, particularly when bike facilities are interrupted, when destinations are located on the same side of the street, or when intersection maneuvers impose high switching or crossing costs. At the same time, residential roads exhibit a more favorable association than general major or minor roads, although their effect remains weaker than segments explicitly equipped with protected bike lanes. This pattern suggests that low traffic riding environments provide an important baseline for e-bike route choice. Residential streets can therefore play a critical role, particularly in settings where route options are limited and riders seek lower stress alternatives.

%Note: trip purpose and profile can be different;

Based on the results of these micro-built environment variables, natural landscape elements do not show a consistently positive association. This suggests that, in the travel context of our study, greenery or scenic aesthetics is not a primary driver of e-bike route choice. Instead, we argue that e-bike riders’ preferences more likely reflect an environment perception mechanism oriented toward connectivity and travel efficiency, rather than purely aesthetic appeal. Specifically, riders appear to place greater value on the legibility and spatial organization of street space, as well as visual cues that indicate stronger network connectivity and more stable riding conditions. In addition, street environments characterized by clear spatial boundaries and continuous urban interfaces may further increase route attractiveness.

Finally, based on the analysis above, we recommend prioritizing protected bike lanes on high speed or high volume corridors to provide reliable protection for e-bike travel. This recommendation is further supported by social evidence that protected bike lanes are perceived not only to increase cycling willingness but also to enhance neighborhood desirability. Such infrastructure may also promote transportation equity by enabling participation from the “Interested but Concerned” group, which is more vulnerable to perceived traffic stress and safety risks \cite{mcneil2015influence}. At the same time, motorists still express concerns about potential impacts of physical buffers on congestion and parking \cite{monsere2014lessons}, highlighting the need to balance safety benefits with implementation feasibility through careful corridor selection, intersection design, and complementary traffic and parking management. Where protected lanes are not feasible due to space constraints, painted lanes remain a meaningful intermediate option. Although less effective than protected infrastructure, they are preferable to no facility and should be implemented primarily on lower scale minor streets, where markings can improve legibility and perceived space allocation. Sidewalk continuity and rideability should be improved along high stress corridors as a practical low-stress option. At the same time, potential conflicts with pedestrians should be explicitly addressed through appropriate design and management measures. Residential streets should be connected into a continuous network. Given their inherently low-traffic environment, micromobility-oriented treatments such as bicycle boulevards can further enhance their benefits.


\subsection{Comparisons between e-bike and bicycle}


%E-bike were found to be associated with higher average numbers of trips on major roads than bicycles \cite{chavis2021bikes}. 

To interpret the e-bike route choice results, it is useful to relate them to prior findings for bicycles and e-scooters. Although these modes operate within similar street networks, differences in vehicle characteristics and typical travel contexts imply that route choice sensitivities may vary across modes. Comparing evidence across bicycles, e-scooters, and e-bikes therefore provides a clear comparative framework to identify shared behavioral tendencies as well as mode-specific responses. 

We focus on e-bike and bicycle comparisons in this section. Specifically, evidence for bicycles in this section is drawn from general patterns reported across the existing literature: Compared with e-bike riders, bicycle riders are significantly more sensitive to steep slopes and route complexity (e.g., frequent turns), and show stronger aversion to arterial roads with painted bike lanes. They also exhibit stronger preferences for low-stress facilities and environments, including off-road cycleways, protected bike lanes, and mixed-traffic local streets (e.g., sharrows) \cite{lilasathapornkit2025cycling, chavis2021bikes}. Bicycle riders may overestimate their tolerance for steep slopes after switching to e-bikes \cite{khavarian2024bike}. Note that our empirical analysis does not include bicycle data. As such, our study cannot provide a direct within-sample comparison between bicycle and e-bike riders. Nevertheless, drawing on this contextual evidence, we discuss how our findings on e-bike route choice may complement and extend existing comparative studies by highlighting patterns that are consistent with, or deviate from, previously reported contrasts.

Many of the preference patterns and sensitivities commonly reported for bicycle riders remain statistically significant in our e-bike sample, suggesting that the two groups share broadly similar route choice mechanisms. Specifically, Our findings further support that, similar to bicycle riders, e-bike riders also value lower-stress roads: major roads continue to generate an overall disutility, and e-bike riders consistently avoid shared facilities while favoring protected infrastructure. Overall, we do not observe notable sign reversals in preferences or drastic changes in statistical significance across road types, facility types, or their interactions. This implies that e-bike route choice behavior does not exhibit a fundamental departure from bicycle riders.

Notably, one potential sign difference relative to bicycle evidence may arise for off-street cycleways, for which we obtain a negative association in our e-bike sample. In bicycle route choice studies, off-street cycleways are typically favored because they provide a safer and more comfortable riding environment. For commuting-oriented shared e-bike trips, the features of off-street cycleways, such as weaker connectivity to the street network, indirect alignments, and lower effective travel speeds, may outweigh the benefits of low-stress riding space. This pattern suggests that the observed e-bike trips may prioritize travel efficiency over comfort or perceived safety. Supporting evidence can be found in the speed literature, which highlights the context-dependent nature of e-bike speed advantages: faster e-bike cycling is more likely to be achieved along main streets \cite{khavarian2024bike}, whereas speeds on non-motorized paths (e.g., greenways) are often constrained \cite{langford2015risky}. This may reflect indirect facility geometry (i.e., lower linearity), shared-use conflicts with pedestrians, and user-composition effects (e.g., sport-oriented cyclists), although disentangling these mechanisms is beyond the scope of this study.


Another relevant point concerns how painted bike lanes perform on minor roads. In such lower-scale environments, painted markings may improve legibility and perceived space allocation, which could explain the relatively more favorable attitude toward these facilities. This observation echoes a common claim in the literature that cyclists tend to feel safer on e-bikes than on bicycles \cite{arning2023review}, possibly because motor assistance enables riders to maintain a more consistent speed under more complex conditions. However, our results suggest that such advantages primarily manifest on smaller streets and fail to offset the high perceived traffic stress on wider, multi-lane roads. In other words, within the context of our study, the dynamic advantages and perceived safety improvements associated with e-bikes are not sufficiently strong or consistent to fundamentally alter the need for dedicated infrastructure.

Beyond identifying preference sign reversals, we also examine differences in the magnitude of estimated sensitivities and preference intensities across attributes. Although our dataset does not allow a direct within-sample comparison between bicycle and e-bike riders, the relative magnitudes of estimated effects across attributes within our e-bike model allow us to infer several potentially meaningful distinctions.

1) We find that residential roads exhibit a substantially weaker positive association compared with major/minor roads with protected bike lanes. This pattern is not prominently highlighted in bicycle route choice literature and may imply that residential streets are less attractive for e-bike riders than for bicycle riders. One plausible explanation is speed-related: routes primarily composed of small streets may lead to lower effective travel speeds \cite{khavarian2024bike}, which may be less compatible with the more efficiency-oriented travel context of many e-bike trips.

2) E-bike riders exhibit lower but still present sensitivity to elevation. For bicycles, slope effects become increasingly negative beyond moderate gradients, with steep segments above 10\% showing strong deterrent effects. The e-bike results occupy an intermediate position: slope effects are insignificant at moderate levels but become significantly negative only for steep gradients exceeding 10\%, suggesting that electric assistance mitigates, but does not eliminate, aversion to challenging terrain. This difference may be related to mode-specific riding posture, physical experience, and vehicle form factors, such as body position and vehicle size, which shape how elevation changes are perceived during travel.

%physical effort: the greater physical demands of non-motorized cycling. Without motor support, interruptions and inclines present greater effort and can act as deterrents. vs smoother acceleration, reduced fatigue, and the ability to maintain consistent speed in more complex conditions


\subsection{Comparisons between e-bike and e-scooter}

The evidence for e-scooters in this section is drawn from a Washington, DC study using a comparable modeling framework to this study. Overall patterns for road types and bike facilities are broadly similar. E-scooter users also consistently favor protected facilities. However, e-scooter riders appear to be more tolerant of painted or shared lanes than e-bike riders, while residential roads are relatively more attractive for e-scooters. In addition, off-street cycleways are positively associated with e-scooter route choice, suggesting that e-scooter preferences in this dimension may be closer to bicycle behavior than to e-bike behavior. Regarding intersection-related friction, bicycle studies and our e-bike results both show negative associations with traffic signals, whereas traffic signals do not exhibit statistically significant effects in the e-scooter study.

We interpret these differences as reflecting distinct travel contexts and vehicle characteristics. Typical e-scooter trips are shorter, and users may place lower demands on high-quality on-street facilities along major corridors compared to commuting-oriented e-bike trips. At the same time, e-scooters tend to have lower stability, making interactions with lane changes, overtaking traffic, or heavy vehicles particularly risky. This may explain a stronger preference for residential streets and off-street cycleways that offer low traffic volumes, fewer conflicts, and more slow-speed operating environments. In contrast, e-bikes, with higher speed potential and stronger power assistance, are more likely to be used in commuting contexts where efficiency advantages are realized on higher-class corridors. This can also increase reliance on high-quality cycling infrastructure and elevate sensitivity to intersection-related interruptions.

Micro-built environment effects are also largely consistent across modes. The impacts of features such as sky and walls appear similar between e-bike and e-scooter models. One notable difference is that trees exhibit a positive association for e-scooters. Beyond aesthetic appeal, this may reflect the shading benefit of street trees in reducing heat exposure and improving thermal comfort. This interpretation is plausible given that e-scooter users are typically fully exposed to ambient conditions, and shading may thus provide more salient comfort benefits.

Finally, sensitivity to elevation varies across modes. In the e-scooter study, slope-related variables are largely statistically insignificant, indicating limited sensitivity to elevation changes. When combined with our e-bike results, this suggests that although both modes are electrically assisted, motorization appears to almost eliminate slope deterrence for e-scooters, whereas a non-negligible elevation sensitivity remains for e-bike riders. A plausible explanation is that shared e-bikes in Washington, DC are primarily pedal-assist, meaning that riders still need to provide human effort during climbing, while e-scooters rely on fully motorized propulsion with no pedaling involvement.



\section{Conclusion}



%Aligning infrastructure design play a critical role in supporting broader e-bike adoption and effective micromobility planning.

This study examined shared e-bike route choice in the urban environment of Washington, DC by applying a path size logit model to GPS-based revealed preference data. The model integrates road types, cycling infrastructure, network characteristics, elevation, and micro-built environment features derived from Street View imagery. The results demonstrate strong predictive performance and reveal clear behavioral patterns. E-bike riders prefer shorter and simpler routes, with significant avoidance of longer distances, frequent turns, and signalized intersections. Roadway hierarchy and facility design jointly shape route utility. Major roads generate overall disutility, and shared lanes on major roads are the most deterrent. Protected bike lanes strongly increase route attractiveness on both major and minor roads. In contrast, painted bike lanes exhibit pronounced context dependence, performing poorly on major roads but offering a positive and acceptable option on minor roads. Beyond on-road facilities, bikeable sidewalks show the largest positive association, suggesting that in constrained or high-stress corridors, sidewalks legally open to bicycles can function as a practical low-stress alternative when on-street protection is absent or insufficient. Residential streets also provide a supportive baseline for e-bike travel. Off-street cycleways are negatively associated in this shared e-bike sample, consistent with the interpretation that utilitarian trips may prioritize efficiency over off-street space when such facilities are indirect or weakly connected. Elevation effects are non-linear. Moderate slopes are not systematically avoided, but steep segments above 10\% significantly deter route choice, indicating lower but still present sensitivity to elevation under pedal assist. Overall, our findings suggest that an e-bike-supportive network requires targeted deployment of protected facilities on high-stress major corridors, complemented by context-appropriate painted lanes on lower-scale streets and a connected set of low-stress alternatives. In particular, this includes improving sidewalk continuity and managing pedestrian conflicts where sidewalks serve as a low-stress option, as well as connecting residential streets into continuous low-stress networks through micromobility-oriented treatments such as bicycle boulevards.
%%%%%%%%%%
 

Beyond conventional GIS-based infrastructure variables, this study incorporates micro-built environment features extracted from Street View imagery to capture street-level visual context. The Street View-derived measures provide empirical evidence that micro-scale visual cues are systematically associated with e-bike route choice. In particular, greenery-related elements do not exhibit consistently positive effects, whereas sky visibility, walls, and cars are positively associated. These patterns may reflect riders’ sensitivity to street-level openness, spatial legibility, continuous built edges, and corridor activity, suggesting that perceived riding conditions are shaped not only by physical infrastructure but also by how the environment is visually experienced. Methodologically, our results highlight the value of integrating computer vision–based streetscape measures into behavioral route choice models, offering a practical way to incorporate high-resolution street context into micromobility research and planning.

%role of cycling infrastructure,context-dependent ； underscoring that the effectiveness of different facility types may vary with urban spatial structure, network design, and cycling trip purposes. user profile can be different;

Several limitations of this study should be acknowledged. First, the model does not account for individual-level demographic or socioeconomic characteristics due to data constraints and privacy considerations, which could contribute to unobserved individual preference heterogeneities. Future research could address this limitation by integrating GPS-based trip data with user attributes or survey-based perception data. Second, this analysis focuses on Washington, DC and its surrounding areas. Additional studies across different urban forms and transportation contexts are needed to assess the generalizability of these findings and to further explore how street-level environments influence e-bike route choice. Third, pre-trained computer vision models were used to segment or detect micro-built environment features from Street View images without fine-tuning, which limits the accuracy of the extracted features. Collecting annotated Street View image datasets would enable fine-tuning of these models and improve prediction accuracy within the local study context. Lastly, our analysis focuses on utilitarian trips by removing trips with duplicate nodes or links, ensuring that choice sets could rely solely on observed routes. Future research could examine recreational travel or adopt other route-generation techniques, such as combining observed routes with algorithm‑based synthetic alternative route generation.



\section{Acknowledgments}
We are grateful for the funding support from U.S. National Science Foundation (Award \#2425029). ChatGPT was used to improve the readability and language of the work.  

\newpage


\bibliographystyle{trb}
\bibliography{trb_template}
\end{document}




